COSMU: Complete 3D human shape from monocular unconstrained images

We present a novel framework to reconstruct complete 3D human shapes from a given target image by leveraging monocular unconstrained images. The objective of this work is to reproduce high-quality details in regions of the reconstructed human body that are not visible in the input target. The proposed methodology addresses the limitations of existing approaches for reconstructing 3D human shapes from a single image, which cannot reproduce shape details in occluded body regions. The missing information of the monocular input can be recovered by using multiple views captured from multiple cameras. However, multi-view reconstruction methods necessitate accurately calibrated and registered images, which can be challenging to obtain in real-world scenarios. Given a target RGB image and a collection of multiple uncalibrated and unregistered images of the same individual, acquired using a single camera, we propose a novel framework to generate complete 3D human shapes. We introduce a novel module to generate 2D multi-view normal maps of the person registered with the target input image. The module consists of body part-based reference selection and body part-based registration. The generated 2D normal maps are then processed by a multi-view attention-based neural implicit model that estimates an implicit representation of the 3D shape, ensuring the reproduction of details in both observed and occluded regions. Extensive experiments demonstrate that the proposed approach estimates higher quality details in the non-visible regions of the 3D clothed human shapes compared to related methods, without using parametric models.

==> sec/0_abstract.tex <==
\begin{abstract}
We introduce a novel framework to reconstruct complete, high-quality 3D human shapes from monocular unconstrained images, ensuring high-quality details in all the regions of the reconstructed human body. The proposed work addresses the limitations of existing approaches for reconstructing 3D human shapes from a single image, which cannot reproduce shape details in occluded body regions. The missing information of the monocular input can be recovered by using multiple views captured from multiple cameras. However, multi-view reconstruction methods necessitate accurately calibrated and registered images, which can be challenging to obtain in real-world scenarios.
%
Given a target RGB image and a collection of multiple uncalibrated and unregistered images of the same individual, acquired using a single camera, we propose a novel framework to generate complete, high-quality 3D human shapes. We introduce a novel module to generate 2D multi-view normal maps of the person registered with the target input image. The module consists of body part-based reference selection and body part-based registration. The generated 2D normal maps are then processed by a multi-view attention-based neural implicit model that estimates an implicit representation of the 3D shape, ensuring high-quality details in both observed and occluded regions.
%
Extensive experiments demonstrate that the proposed approach estimates higher quality 3D clothed human shapes from a set of unconstrained images compared to related methods, without the use of parametric models.
\end{abstract}


==> sec/1_introduction.tex <==
\section{Introduction}
\label{sec:1_intro}
Democratizing the creation of high-quality human avatars is essential to unlock a wide range of immersive technologies including self-representation in the metaverse, virtual conferencing, and virtual try-on. Realistic human avatars are crucial in these applications, making 3D human reconstruction a prominent topic in computer vision and graphics. Research focuses on finding practical solutions to replace existing sophisticated multi-view systems for 3D reconstruction, which are inaccessible to the general community. Single-view 3D human reconstruction methods have been developed to reconstruct 3D human shapes using a simple and cost-effective set-up, such as a single camera. 
\\Recent methods~\cite{saito2019pifu,he2020geopifu,alldieck2022photorealistic,corona2023structured,he2021arch++,huang2020arch} use neural implicit models to estimate 3D human shapes with high-quality details in visible regions from single RGB images. These works fail to reproduce fine detail in invisible regions of the input image, resulting in overly smooth reconstruction.
%
\\To tackle this problem, solutions extend single-view to multi-view reconstruction, using multiple images of various orientations of the human body~\cite{yu2023multi,li2022detailed,zins2021data,zins2023multi,cao2023sesdf}. Multi-view methods represent details across the entire body but require calibrated cameras and registered images, with the subject in the same pose and clothing. Systems to capture such images are inaccessible to the general community in real-world scenarios, significantly limiting reproducibility.
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/intro.pdf}
\caption{COSMU reconstructs complete, high-quality 3D human shape from a target RGB input by leveraging a set of monocular images collected from various scenarios, including monocular video (a), images with different poses (b) and clothing (c).}
\label{fig:introduction}
\end{figure}
%
% \\Other works estimate the invisible part of the body from the input image either by using deep learning frameworks~\cite{saito2020pifuhd} or by estimating and fitting a parametric model to the input~\cite{ICONCVPR2022,xiu2023econ}. Only an additional view of the body is estimated by these approaches, which is not sufficient to represent the whole body, therefore failing to reproduce fine detail in all the shape regions. In addition, the accuracy of the estimation of the invisible region is influenced by the generative power of the network and subjected to noise. Parametric models also struggle to represent clothes. Therefore, the details of invisible regions are still significantly smoother than the ones obtained by multi-view approaches. 
%
\\Recent works~\cite{zhu2022mvp, yu2022multiview,huang2022unconfuse,zheng2021pamir,chen2022crosshuman} reconstruct humans from a single target image by leveraging multiple monocular unconstrained images. We define images as unconstrained if camera calibration parameters are not known (uncalibrated) and the images were captured at different time instances resulting in pose and clothing variations without spatial alignment (unregistered). These methods directly fuse features from multiple images, which is a challenging task since diverse views and poses must be fused into a single coherent reconstruction~\cite{zhu2022mvp}. They rely on parametric models and cannot use images of the person in different clothing.
%
\\We propose COSMU, a novel framework that reconstructs COmplete high-quality 3D human Shape from Monocular Unconstrained images. Our objective is to reconstruct a 3D human shape with high-quality details from a single RGB image by leveraging a collection of unconstrained images of the subject without the use of parametric models.
%
\\COSMU first simulates the multi-view scenario used by the multi-view reconstruction approaches from a collection of unconstrained images, with the subject in different poses and clothing and without camera calibration or corresponndences. 
%
To achieve this, we present a novel pipeline that applies an optimization-based algorithm to select, from the set of unconstrained images, $N_{r}$ references for each $N_{p}$ body part of the target image following an orientation-visibility-similarity criteria. 
%
% The orientation angle between the target 3D pose and each selected reference is also retrieved. 
A neural implicit model generates a coarse point cloud $\zeta_t$ of the target and of each selected reference $\zeta_{ref}$. The 3D points of these point clouds are classified into $N_{p}$ body parts using a novel pixel-aligned neural network. The corresponding reference body part selected for a specific target part is registered to it. To obtain $N_r + 1 $ views of the subject, 2D normal maps are generated from the registered point clouds.  
%
The multi-view scenario is simulated and the 2D normal maps are processed by an attention-based implicit model that estimates the implicit function $f_f$ of the complete, high-quality shape. 
%
COSMU generates 2D multi-view normal maps instead of RGB images because the reference images are not constrained to have the same clothing as the target and RGB values for 3D points do not have to be estimated.
\\
Extensive experiments show COSMU's ability to reconstruct complete, high-quality 3D human shapes from monocular images taken from various scenarios, including monocular videos (\cref{fig:introduction}a), images with different poses and same clothing (\cref{fig:introduction}b)  and images with different poses and clothing (\cref{fig:introduction}c). Thanks to the flexibility in creating the reference set, COSMU represents a significant advance for high-quality 3D avatar reconstruction.
\\The contributions presented in this paper include:
\begin{itemize}[noitemsep]
    \item A novel framework to reconstruct complete, high-quality 3D human shapes from a single RGB image by leveraging a set of monocular uncalibrated and unregistered images without the use of parametric models.
    \item A novel pipeline comprising reference selection and body part registration to simulate a multi-view scenario from a collection of unconstrained images.
    \item Improved performance for human shape reconstruction compared to state-of-the-art methods.
\end{itemize}


==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:5_conclusion}
We introduce a novel framework to reconstruct complete, high-quality 3D human shapes from a single RGB image by leveraging a collection of monocular unconstrained images without using parametric models. We first developed a novel multi-view scenario simulation module to generate a set of registered 2D normal maps of the target subject. An implicit function that represents the 3D shape of the subject is then estimated by a multi-view attention-based neural implicit model. The evaluation demonstrates that the proposed approach can be applied in various scenarios. Significantly higher quality details are reproduced in hidden regions compared to state-of-the-art works. As future works, a solution to enhance the quality of smaller body regions will be investigated and the approach will be extended to reconstruct temporally-coherent dynamic shapes.

==> sec/evaluation_v2.tex <==
\section{Experiments}
\label{sec:4_experiments}
\begin{figure*}[t!]
\centering
\includegraphics[width=0.95\linewidth]{figures/ablation1.pdf}
\caption{Qualitative comparisons between 3D shapes from THuman3.0~\cite{deepcloth_su2022} reconstructed by changing the energy optimization process to select reference images. Front, back and side views of the shapes are illustrated.}
\label{fig:ablation_energy}
\end{figure*}
We conduct a comprehensive evaluation of COSMU for the task of 3D human shape reconstruction from a single image by leveraging a collection of monocular unconstrained images of the same individual. The neural models of the framework are trained with THuman2.0 dataset~\cite{tao2021function4d}, which comprises 524 high-resolution surfaces. We render 360-degree view images around each surface, which serves as input data. For the quantitative and qualitative evaluation, we use the THuman3.0 dataset~\cite{deepcloth_su2022}, which consists of 20 individuals, each captured in various poses. For each pose, we render 360-degree views of the subject and we apply the reference selection to select the $N_p \times N_r$ references among the images of the subject in different poses, excluding the target one. We evaluate the reconstruction accuracy with three quantitative metrics: the normal reprojection error~\cite{saito2019pifu}, the average point-to-surface Euclidean distance (P2S) and the Chamfer distance (CD), expressed in cm. We further test COSMU with real data collected from various scenarios, including monocular videos (People-Snapshot~\cite{alldieck2018video}, iPER~\cite{lwb2019} datasets) or images of people in different poses and clothing from the Internet, demonstrating its superiority over related works to reconstruct complete, high-quality 3D human shapes from both synthetic and real images without using parametric models (\cref{ssec:comparison_cosmu}). We set $N_p=10$ and $N_r=3$. See supplementary for additional implementation details.
\subsection{Ablation Studies}
\label{ssec:ablation}
\textbf{Energy function for reference selection}:
We conduct an ablation study on the criteria used for selecting the $N_p \times N_r$ references in the body part-based reference selection. The variants explored are: (i) \textbf{Random}: no criteria are applied. $N_p$ references are randomly selected for each group; (ii) \textbf{Only} $\mathbf{b_p}$: only the body part pose similarity is considered; (iii) \textbf{Only} $\mathbf{o}$: the body orientation angle is the only criterion used; (iv) \textbf{Only} $\mathbf{v_p}$: only the body part visibility is considered; (v) $\mathbf{o + v_p}$: the body part pose similarity is excluded; (vi) $\mathbf{o + b_p}$: the body part visibility is omitted; (vii) $\mathbf{v_p + b_p}$: the orientation angle is not used.
\\As illustrated in~\cref{fig:ablation_energy} and supported by the quantitative results of~\cref{tab:ablation_energy}, the 3D shapes obtained with COSMU exhibit fewer artifacts and finer details. The reference selection plays a crucial role in selecting the most suitable references to facilitate the body part-based registration. Omitting any of the criteria in the energy optimization influences the selection of references, leading to suboptimal choices and, consequently,  deteriorating the body part-based registration accuracy and introducing artifacts in the reconstruction.
\begin{table}[!]
\caption{Quantitative evaluation of the application of different energy optimization processes to select reference images.}
\centering
% \renewcommand\arraystretch{1.1}
% \setlength{\tabcolsep}{4pt}
\resizebox{0.58\linewidth}{!}{\input{tables/ablation1}}

\label{tab:ablation_energy}
\end{table}
\\\textbf{Body part-based registration effectiveness}: Directly using $N_r$ selected references for the multi-view reconstruction deteriorates the performance since fusing different poses is challenging in the absence of known correspondences. To avoid this, we introduce a novel body part-based registration method to simulate a multi-view scenario. To prove its effectiveness, we modify the algorithm for registering the $N_p \times N_r$ coarse reference point clouds $\zeta_{ref}$ to the target $\zeta_t$:
\begin{itemize}[noitemsep]
    \item\textbf{No Reg}: To demonstrate the efficiency of registering the reference point clouds to the target, we omit the body part-based registration step. We adjust the reference selection to select only $N_r$ references by averaging over $p$ the criteria $v^p_g$ and $b^p_g$ in ~\cref{eq:energy}.
    \item\textbf{Non Rigid}: Instead of applying rigid registration among the correspondent body parts of the target and reference point clouds, we apply the state-of-the-art work~\cite{li2022DeformationPyramid} to perform non-rigid registration between the point clouds. We use $N_r$ references as in \textbf{No reg}.
    \item\textbf{Average}: COSMU registers a target body part with the corresponding body part of a reference selected specifically for that body part. In this configuration, we select only $N_r$ references as in \textbf{No reg} and register all the body parts of the single reference for each group. 
    \item\textbf{No RGB}: The body part classification model $f_{\zeta}$ processes a concatenation of 2D RGB images and segmentation masks. To demonstrate the advantages of using these data, we train and test $f_{\zeta}$ with only segmentation masks.
    \item\textbf{No Segm}: we train and test $f_{\zeta}$ with only RGB images.
\end{itemize}
\begin{table}[t]
\caption{Quantitative evaluation of the application of different configurations of the body part-based registration algorithm.}
\centering
% \renewcommand\arraystretch{1.1}
% \setlength{\tabcolsep}{4pt}
\resizebox{0.8\linewidth}{!}{\input{tables/ablation2}}

\label{tab:bodypart}
\end{table}
We apply these configurations to generate 2D multi-view normal maps used by the multi-view attention-based implicit model to reconstruct 3D human shapes. Quantitative (\cref{tab:bodypart}) and qualitative results (\cref{fig:ablation_shape}) show that COSMU configuration is the most effective. Multi-view reconstruction requires registered input since pixel-alignment across different views can be incorrect with unregistered views. 
\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\linewidth]{figures/ablation2_shape.pdf}
\caption{Qualitative comparisons between 3D shapes from THuman3.0~\cite{deepcloth_su2022} reconstructed from 2D normal maps generated using different configurations of the body part-based registration algorithm. Front, back and side views of the shapes are shown.}
\label{fig:ablation_shape}
\end{figure*}
Estimating correspondences between point clouds is challenging and the non-rigid registration cannot produce reliable results. Selecting $N_p$ references for each body part facilitates the body part registration compared to using a single reference. Leveraging RGB and segmentation masks improves the body part classification since the model learns both
semantic and appearance information.
\subsection{Comparisons}
\label{ssec:comparison_cosmu}
We conduct a comparative evaluation of COSMU against related works that reconstruct complete 3D human shapes from monocular RGB images. We evaluate MVP-Human~\cite{zhu2022mvp} (MVP) and Multi-Pamir~\cite{zheng2021pamir} that reconstruct 3D shapes from unconstrained images leveraging SMPL~\cite{SMPL:2015} in the process. The same $N_r=3$ images selected in the ablation study (\cref{ssec:ablation}) are used as additional views. We then evaluate approaches that estimate an unseen view of the subject directly from the target image (PiFU-HD~\cite{saito2020pifuhd}, ICON~\cite{ICONCVPR2022} and ECON~\cite{xiu2023econ}). Since these methods use two views in the reconstruction, we train and evaluate COSMU-2 by selecting $N_r=1$ reference ($\theta_c=180\degree$). This demonstrates the effect of using a lower number of references in the reconstruction. We then compare COSMU with PiFU~\cite{saito2019pifu} and SuRS~\cite{SuRSECCV2022}, which process a single view without any information on hidden regions. 
%
We evaluate $f_{c}$ (Baseline) that reconstructs the coarse target point clouds $\zeta_t$ without applying any registration or leveraging additional views. This is equivalent to testing COSMU with $N_r=0$. We train all the approaches with THuman2.0~\cite{tao2021function4d}.
%
\\\textbf{Quantitative evaluation} is conducted with the 3D shapes reconstructed from single images of THuman3.0~\cite{deepcloth_su2022} and the results presented in~\cref{tab:comparisons} demonstrate the superiority of COSMU across all the considered metrics.  The best scores overall are highlighted in red while the best scores for approaches that use 2 views are blue. COSMU achieves the highest accuracy among all the tested methods while COSMU-2 outperforms approaches that rely on 2 views, demonstrating the benefit of leveraging views from 2D images rather than estimating them from the input. The worst results are obtained with single-view approaches.
\begin{table}[t!]
\caption{Quantitative comparisons with related works for 3D human reconstruction from a single or multiple views.}
\centering
% \renewcommand\arraystretch{1.1}
% \setlength{\tabcolsep}{4pt}
\resizebox{0.55\linewidth}{!}{\input{tables/comparisons_v2}}
\label{tab:comparisons}
\end{table}
\textbf{Qualitative results: }\cref{fig:comparisons} illustrates the 3D shapes reconstructed applying the considered methods across several scenarios. The first set of shapes is reconstructed by leveraging a collection of images of the same individual in different poses from THuman3.0~\cite{deepcloth_su2022}. 
%
The target and references of the second set are taken from the same monocular video of a person rotating from People-Snapshot~\cite{alldieck2018video}. 
%
In the third set, random images of a person in different poses and clothing are selected from the Internet. 
%
The target image of the fourth set is a single frame of a monocular video where the human body is not entirely seen. The references are taken from other monocular videos of iPER~\cite{lwb2019} where the subject wears random clothing and the entire body is seen. These two scenarios represent the most challenging task due to the significant difference between the reference images and the target one.
\\In all the considered scenarios, COSMU consistently reproduces high-quality details in all the regions of the 3D shape, significantly outperforming related works. MVP struggles to reproduce details and introduces noise when the subject is wearing different clothing in the references ($3^{rd}$  and $4^{th}$ set). ECON can represent details on unseen parts of the model but at a notably lower quality compared to COSMU and COSMU-2, which are the only two approaches capable of reconstructing the hood on the back of the jumper. COSMU-2 exhibits artifacts and excessive smoothing on the sides of the shapes, demonstrating the benefit of leveraging references showing the entire body. The shapes reconstructed by ECON and MVP are influenced by the incorrect estimation of SMPL, resulting in an unnatural bending of the 3D body ($2^{nd}$ and $4^{th}$ set). SuRS reproduces high-quality details in the regions that are visible in the image, with excessive smoothed reconstruction in other regions.
\begin{figure*}[!]
\centering
\includegraphics[width=\textwidth,height=0.99\textheight,keepaspectratio]{figures/comparisons.pdf}
\caption{Qualitative examples of 3D shapes reconstructed in several scenarios. Static images are from THuman3.0~\cite{deepcloth_su2022}; monocular videos are from People-Snapshot~\cite{alldieck2018video} and iPER~\cite{lwb2019};  random images are from the Internet. Front, back and side views are shown.}
\label{fig:comparisons}
\end{figure*}
\\\textbf{Limitations}:
%
COSMU's ability to reconstruct high-quality details is contingent on the availability of reference images. COSMU cannot reproduce high-quality details in a region that is not visible in the reference images. 
%
Performance deteriorates when the reference images significantly differ from the target. See supplementary for a study on choosing references with varying degrees of similarity to the target. In some examples, COSMU cannot reproduce the same high-quality level of details in small regions of the body, such as the face and hands. The registration algorithm struggles to register small body parts while the multi-view transformer struggles to fuse multiple views of those regions.

==> sec/methodology_v2.tex <==
\section{3D human shape reconstruction from monocular unconstrained images}
\label{sec:3_methods}
\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures/arch.pdf}
\caption{COSMU framework: given a single RGB image as input and a collection of monocular unconstrained images, a {\color{blue_mod}multi-view scenario simulation module}, which consists of part-based reference selection and registration, is first applied to generate registered multi-view 2D normal maps of the subject in the same pose. An implicit function $\hat{s}_f$ is then estimated by processing these normal maps with a {\color{red_mod}multi-view attention-based neural implicit model}. The 3D mesh is reconstructed via marching cube.}
\label{fig:arch}
\end{figure*}
We introduce a novel framework that reconstructs COmplete, high-quality 3D human Shape from Monocular Unconstrained images (COSMU). We consider a 3D human shape to be complete if it contains high-quality details in all the regions of the body. A single image lacks the necessary information to reproduce details across the entire body, which can instead be extracted from multi-view images. In contrast to multi-view reconstruction, which requires calibrated and registered images captured with inaccessible systems, COSMU reconstructs complete, high-quality 3D shapes from single images by leveraging a collection of uncalibrated and unregistered images, referred to as unconstrained images. The input is a target image $I_t$ of a person together with multiple views of the same person in various poses and either same or different clothes, from which we extract body part detail occluded in the target view. As shown in~\cref{fig:arch}, COSMU, given a set $\mathbf{U}=\{I^m_u\}^{N_u}_{m=1}$ of $N_u$ monocular unconstrained images, simulates the multi-view scenario of traditional multi-view methods using a novel module that employs body part-based reference selection and registration to create 2D multi-view normal maps registered with the target input. A multi-view attention-based implicit model processes the normals to regress the implicit representation $f_{f}$ of the complete, high-quality 3D shape.
\subsection{Multi-view scenario simulation module}
Directly processing unconstrained images with a multi-view neural model deteriorates the performance due to their unregistered nature (\cref{ssec:ablation}). To address this, we propose a novel pipeline that simulates a multi-view scenario in which the multi-view images represent various orientations of the subject in the same body pose. Given a target image $I_{t}$, we select $N_{p} \times N_{r}$ references $\left\{\{I_{ref}^{\{p,r\}}\}^{N_p}_{p=1}\right\}^{N_r}_{r=1}, I_{ref} \in \mathbf{U}$, from the collection $\mathbf{U}$ of unconstrained images applying a body part-based reference selection. 2D registered multi-view normal maps are then created by registering references to the target input via body part-based registration. Set notation is dropped for simplicity.
\\\textbf{Body part-based reference selection: }To improve the body part-based registration, we select references observed from complementary orientations and with body part poses similar to the corresponding target body part ones. $N_r$ references are selected for each $N_p$ body part of the target $I_t$ via energy optimization following an orientation-visibility-similarity criteria.  Semantic masks $M$ and 3D poses $P$ are extracted from the input images. To ensure that the entire body is represented in the selected references, we first divide the $N_u$ unconstrained images into $N_r$ groups based on the full-body orientation angle $\theta_u$ computed between the reference $P_u$ and the target $P_t$ 3D poses with the Rodrigues rotation formula. Each group contains a variable number $N_g$ of unconstrained images $I^g_u, g \in [1,\ldots,N_g]$. $N_p$ references $I_{ref}$ are selected from each group following 3 criteria:
\\\textbf{1.} Body orientation angle: for a complete view of the body, the selected images should complement each other in the body orientation. An orientation metric is introduced to enforce the selection of images in which the body orientation is closer to the central angle $\theta^r_c$ of the $r^{th}$ group:
\begin{equation}
\label{eq:orientation}
    o_g=|\theta^r_c-\theta_u|,\quad \theta^r_c=r\cdot\frac{360}{N_r+1},\quad r\in[1,...,N_r]
\end{equation}
\\\textbf{2.} Body part visibility: every body part should be visible in the selected references to have a complete view of the body. We use a visibility metric that counts the total number of pixels $N_M$ of each body part $p$ in the semantic masks $M$.
\begin{equation}
\label{eq:visibility}
    v_g^p=N^p_M,\quad p\in[1,...,N_p]
\end{equation}
\\\textbf{3.} Body part pose similarity: similarity between each body part of $I^g_u$ and the corresponding body part of $I_t$ is evaluated as 3D Euclidean distance between the corresponding 3D bones of $P_g$ and $P_t$, ensuring spatial consistency:
\begin{equation}
\label{eq:similarity}
    b_g^p=||P^p_t-P^p_g||,\quad p\in[1,...,N_p]
\end{equation}
$o_g=o(I^g_u), v^p_g=v^p(I^g_u), b^p_g=b^p(I^g_u)$ for the $g^{th}$ image $I^g_u$ of the $p^{th}$ body part.% in the $r^{th}$ group. 
\\$N_p$ references $I_{ref}$ are selected by minimizing the energy $E^p_{g}$ over the $N_g$ images $I^g_u$ for each body part $p$:
\begin{equation}
\label{eq:energy}
\begin{gathered}
   I_{ref}=\argmin_{g}(E^{p}_{g})\\
  \resizebox{0.65\hsize}{!}{$  E^{p}_{g}=idx_{min}\left(o_g\right)+idx_{max}\left(v^p_g\right)+idx_{min}\left(b^p_g\right)$}
\end{gathered}
\end{equation}
$idx_{min}$ indicates the position $idx$ of the $g^{th}$ image $I^g_u$ in the arrays created by sorting all the $N_g$ images with respect to their specific metric $K=o_g, v_g^p, b_g^p$. $idx_{max}$ sorts the array in inverse order:
\begin{equation}
\begin{gathered}
   \resizebox{0.75\hsize}{!}{$
   idx_{min}(K)= \idx_{I^g_u} \{I^1_u,\ldots,I^{N_g}_u\}, \resizebox{0.28\hsize}{!}{${K(I^1_u) \leqslant \ldots \leqslant K(I^{N_g}_u)}$}$}\\
  \resizebox{0.75\hsize}{!}{$ idx_{max}(K)= \idx_{I^g_u} \{I^1_u,\ldots,I^{N_g}_u\}, \resizebox{0.28\hsize}{!}{${K(I^1_u) \geqslant \ldots \geqslant K(I^{N_g}_u)}$}$}
\end{gathered}
\end{equation}
$N_p \times N_r$ references are selected by repeating the body part-based reference selection for every group.
\\\textbf{Body part-based registration: }
To simulate the multi-view scenario given the selected $N_p \times N_r$ references, we register each 3D reference body part to the corresponding 3D body part in $I_t$. This process begins with the reconstruction of a coarse point cloud $\zeta_t$ for $I_t$ and for each of the $N_p$ reference images $I_{ref}$ previously selected for the $N_r$ groups ($\zeta_{ref}$). We use a neural implicit model $f_{c}$ comprising of a U-Net that increases the resolution of the input features $\phi(I)$ as in~\cite{SuRSECCV2022}. The coarse implicit function is estimated as:
\begin{equation}
\label{eq:coarse_point}
\hat{s}_c=f_{c}\Bigl(\phi\bigl(\pi(I)\bigr),z(x)\Bigr), \quad \hat{s}_{c}\in \mathbb{R}
\end{equation}
where $I$ is either $I_t$ or $I_{ref}$, $\pi$ represents the orthographic projection of 3D points $x$ into the input images $I$ and $z(x)$ is the depth of $x$. $f_c$ is trained with:
\begin{equation}
    \mathcal{L}_{c}=\frac{1}{N}\sum_{i=1}^{N}\left|f_{c}(X^i_{c})-f_{c}^{gt}(X^i_{c})\right|^2 + \left|I-I_{HR}\right|
\end{equation}
where $X^i_{c}=(\phi^i(\pi(I)),z(x))$, $N$ is the number of points in space and $I_{HR}$ is the up-sampled ground-truth version of $I$ used to train the U-Net feature extractor.
\\We then retrieve 3D body parts by classifying each 3D point $x_{\zeta}$ of the point clouds $\zeta_{t/ref}$ with a novel pixel-aligned classification network $f_{\zeta}$. An image feature embedding $\phi(I||M)$ is extracted from the concatenation between the input RGB image and its semantic mask $M$. Each $x_{\zeta}$ is projected using orthographic projection $\pi$ onto the input $I||M$ and indexed to $\phi(I||M)$. An MLP processes this embedding to estimate the body part $\hat{s}_{\zeta}$ to which $x_{\zeta}$ belongs:
\begin{equation}
    \label{eq:part_class}
    \hat{s}_{\zeta}=f_{\zeta}\left(\phi(\pi(I||M)),z(x_{\zeta})\right),\quad \hat{s}_{\zeta}\in [1,...,N_p]
\end{equation}
$N_p$ 3D body parts $\upsilon_{ref}$ are defined for each reference point cloud as well as for the target $\upsilon_t$. Next, the specific $p^{th}$ body part $\upsilon_{ref}$ selected for the corresponding $p^{th}$ target body part $\upsilon_t$ is registered with it as $\upsilon_{reg}=R(\upsilon_{ref})+ T $,
where $R$ is the rotation and $T$ the translation computed via rigid registration. For each group, the registered $N_p$ body parts are combined to create a point cloud $\zeta_{f}$. $N_r$ point clouds $\zeta_{f}$ registered with $\zeta_t$ are generated, rotated by their $\theta_u$ and, together with $\zeta_t$, used to retrieve $N_r +1$ 2D normal maps $S_v$, one for each view $v \in [1,\ldots,N_r+1]$. Normal maps are generated instead of RGB images to avoid the estimation of color values for each 3D point of $\zeta_{t/ref}$ and to allow different clothing in the references. Directly fusing the registered point clouds to obtain the 3D shape is challenging since correspondences are unknown. 
We train $f_{\zeta}$ with a Mean Squared Error $MSE$ loss:
\begin{equation}
    \mathcal{L}_{part}=\frac{1}{N}\sum_{i=1}^{N}\left|f_{\zeta}(X^i_{\zeta})-f_{\zeta}^{gt}(X^i_{\zeta})\right|^2
\end{equation}
where $X^i_{\zeta}=\Bigl(\phi^i\bigl(\pi(I||M)\bigr),z(x_{\zeta})\Bigr)$
\subsection{Multi-view implicit representation}
Neural implicit models have proven to be efficient in reproducing high-quality details in reconstructed 3D shapes. This is attributed to the characteristic of the implicit function that does not discretize the 3D space like other representations~\cite{saito2019pifu}. Leveraging multiple views to learn the implicit representation further enhances the quality of the reconstruction, as it enables the incorporation of information about the entire body. Concatenating features from multiple images is a suboptimal approach because it imposes an order on the views~\cite{zins2021data}. Fusion approaches based on statistics have been proposed~\cite{gardner2019classifying,su2015multi} but their pooling operation causes a loss of information regarding the individual view contributions. Inspired by~\cite{zins2021data}, we propose to fuse the features extracted from the multi-view 2D normals using an attention-based architecture. An attention score is computed for each view $v$ based on the compatibility of a query with a corresponding key, resulting in the generation of $N_{r}+1$ features. Each of these features contains the original information from the corresponding view, merged with the information from all the other views. An MLP then models a pixel-aligned implicit function $f_f$ to learn the occupancy value  $\hat{s}_f$ of the 3D points in space:
\begin{equation}
\label{eq:final_estimation}
\hat{s}_f=f_f\left(A\left(\phi_v(\pi(S_v)),z(x)\right)\right),\quad \hat{s}_f \in \mathbb{R}
\end{equation}
where $\phi_v$ are the feature extracted from each view $v$ of the surface normal $S_v$, $\pi$ indicates the pixel-alignment between the  3D points of the space and each $\phi_v$, $A$ is the attention operation and $z(x)$ is the depth value of the 3D points $x$.  We train the multi-view architecture with an MSE loss:
\begin{equation}
    \mathcal{L}_{f}=\frac{1}{N}\sum_{i=1}^{N}\left|f_{f}(X^i_{f})-f_{f}^{gt}(X^i_{f})\right|^2
\end{equation}
where $X^i_{f}=A\left(\phi_v^i(\pi(S_v)),z(x^i)\right)$.
\\\textbf{Inference:} $N_p \times N_r$ references are selected from the collection of unconstrained images. $N_r+ 1$ 2D normal maps are generated using body part-based registration to simulate a multi-view scenario with registered views of the subject. The normals are processed by the multi-view attention-based model to estimate the implicit representation. The 3D mesh is reconstructed via marching cube~\cite{lorensen1987marching}.
\\To achieve pixel-alignment through projection, multi-view works require the parameters of calibrated cameras in specialized capture systems. In COSMU, instead of using the camera projection matrix for pixel-alignment, 3D points of the space are rotated by $\theta_u$ computed by the multi-view scenario simulation module and projected onto the images using an identity matrix. 
%
Existing approaches create the inference 3D grid centered at the origin. If the subject is not centered in the input images, the multi-view pixel-alignment of COSMU is inaccurate since the same rotated 3D point may not be projected in the corresponding pixel in each view. To tackle this, we set the boundary limits of the 3D grid as the boundaries of the coarse point cloud $\zeta_t$, ensuring multi-view pixel-alignment.


==> sec/pseudocode.tex <==
\begin{algorithmic}[1]


\State Retrieve $\zeta_t$ from $I_t$ by estimating $\hat{s}_{c}$ with~\cref{eq:coarse_point}
\State Retrieve $\{\upsilon^p_t\}^{N_p}_{p=1}$ of $\zeta_t$ by estimating $\hat{s}_{\zeta}$ with~\cref{eq:part_class}
\State Create 2D normal map $S_0$ from $\zeta_t$
% \COMMENT $N_u$ unconstrained images $I_u$ are clustered into $N_r$ groups considering their orientation angle with the target image
\For{i = 1:$N_u$ (for all the unconstrained images)}
\State Add $I^i_u$ to a group $G^r$  with~\cref{eq:grouping} as: $G^r=\{I^g_u\}^{N_g}_{g=1},\quad g \in [1,\ldots,N_g],\quad r \in [1,\ldots,N_r]$
\EndFor


\For{$r$ = 1:$N_r$ (for all the groups)}


% \COMMENT $N_p$ references images $I_{ref}^{p,r}$ are selected for each body part for the $r^{th}$ group  via body part-based reference selection
\State $\{I^{\{p,r\}}_{ref}\}^{N_p}_{p=1}$ =\Call{ReferenceSel}{$\{I^{\{g,r\}}_{u}\}^{N_g}_{g=1}$}
% \COMMENT The selected $N_p \times N_r$ references images $\{\{I^{p,r}_{ref}\}^{N_p}_{p=1}\}^{N_r}_{r=1}$  are processed by the body part-based registration to estimate a 2D normal maps $S_v$ registered with the target input.
\State $S_r=$\Call{PartReg}{$\{I^{\{p,r\}}_{ref}\}^{N_p}_{p=1}, \{\upsilon^p_t\}^{N_p}_{p=1}$}
\EndFor
\State Estimate $\hat{s}_f$ with $f_f$ from the obtained $S_v=\left\{S_0,\{S_r\}^{N_r}_{r=1}\right\}, v \in [1, \ldots, N_r+1]$ with~\cref{eq:final_estimation}
\Statex



\Function{ReferenceSel}{$I_u$} 
\For{p = 1:$N_p$ (for all the body parts)}
\For{g = 1:$N_g$ (for all the images of a specific group)}
\State Compute $o_g$ with~\cref{eq:orientation}
\State Compute $v_g^{p}$ with~\cref{eq:visibility}
\State Compute $b_g^{p}$ with~\cref{eq:similarity}
\EndFor
\For{K in $[o, v^p, b^p]$:}
\If{$K==o$ or $K==b^p$:}
    \State Sort $\{I^g_u\}^{N_g}_{g=1} \quad \rightarrow \quad K=\{I^1_u,...,I^{N_g}_{u}\},\quad K(I^1_u) \leqslant \ldots \leqslant K(I^{N_g}_u)$.
\Else
    \State Sort $\{I^g_u\}^{N_g}_{g=1}\quad \rightarrow \quad K=\{I^1_u,...,I^{N_g}_{u}\},\quad K(I^1_u) \geqslant \ldots\geqslant K(I^{N_g}_u)$.
\EndIf
\EndFor
\State $I^{p}_{ref}=\argmin_{g}(E^{p}_{g})$ with~\cref{eq:energy} where $E^p_g=\idx_{I_u^g}(K=o)+\idx_{I_u^g}(K=v^p)+\idx_{I_u^g}(K=b^p)$
\EndFor
\State\Return $\{I^{p}_{ref}\}^{N_p}_{p=1}$
\EndFunction
\Statex
\Function{PartReg}{$I_{ref}, \upsilon_t $} 
\For{p = 1:$N_p$ (for all the body parts)}
\State Retrieve $\zeta^p_{ref}$ from $I^p_{ref}$ by estimating $\hat{s}_{c}$ with~\cref{eq:coarse_point} 
\State Retrieve $\upsilon^p_{ref}$ from $\zeta^p_{ref}$ by estimating $\hat{s}_{\zeta}$ with~\cref{eq:part_class}
\State Register $\upsilon^p_{ref}$ with $\upsilon^p_t$ as $\upsilon^p_{reg}=R(\upsilon^p_{ref})+ T $ 
\EndFor
\State Combine the $N_p$ registered body parts $\{\upsilon^p_{reg}\}^{N_p}_{p=1}$ into a point cloud $\zeta_f$
\State Create 2D normal map $S$ from the registered point cloud  $\zeta_f$
\State\Return $S$
\EndFunction




% Three sorted vectors are obtained, one for each metric.  
%     % \begin{itemize}
%     \\$\bullet$ vector $o=[r_1, r_3, r_2,..., r_4],\resizebox{0.4\hsize}{!}{$o^{r_1} \leqslant o^{r_3} \leqslant o^{r_2} \leqslant o^{r_4}$}$
%     \\$\bullet$ vector $b=[r_2, r_1, r_4,..., r_3],\resizebox{0.4\hsize}{!}{$ b^{r_2} \leqslant b^{r_1} \leqslant b^{r_4}  \leqslant b^{r_3}$}$
%     \\$\bullet$ vector $v=[r_3, r_1, r_2,..., r_4],\resizebox{0.4\hsize}{!}{$ v^{r_3} \geqslant v^{r_2} \geqslant v^{r_1} \geqslant v^{r_4}$}$
% \State Compute $r^j_k$ with~\cref{eq:energy}.
% \\$r^j_k=\argmin_{r}\left(E^{j}_{k}(r)\right)=r_1$ since $min\left(E^{j}_{r}(r)\right)=2$ \rightarrow $E^j_k(r_1)=2 \rightarrow  idx_{min}(o^{r_1})=0 + idx_{max}(v^{r_1})=1 + idx_{min}(s^{r_1})=1$; 






% \State Divide $N_M$ reference images in $N_R$ parts
% \State Extract feature vectors of reference image parts $\phi^r(I_{ref}^m)$
% \State Extract feature vectors of LR input $\phi(I_{LR})$
% \State Divide $\phi(I_{LR})$ into $N_C$ subvectors $\rightarrow \{\phi^c(I_{LR})\}^{N_C}_{c=1}$ 

% \For{m = 1:$N_M$ (for all the references)}

\end{algorithmic}


==> tables/ablation1.tex <==
\begin{tabular}{c|cccc}

\multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\textbf{Random}}   & \multicolumn{1}{c|}{\textbf{Only} $\mathbf{b_p}$} & \multicolumn{1}{c|}{\textbf{Only} $\mathbf{o}$}    & \multicolumn{1}{c}{\textbf{Only} $\mathbf{v_p}$} \\ \hline
\multicolumn{1}{c|}{\textbf{CD}}     & 1.485              & 1.441               & 1.421                & 1.410               \\ 
\multicolumn{1}{c|}{\textbf{Normal}} & .1683              & .1598               & .1641                & .1654               \\ 
\multicolumn{1}{c|}{\textbf{P2S}}    & 1.424              & 1.415               & 1.403                & 1.406               \\
\hline
            \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{$\mathbf{o + v_p}$} & \multicolumn{1}{c|}{$\mathbf{o + b_p}$ } & \multicolumn{1}{c|}{$\mathbf{v_p + b_p}$} & \multicolumn{1}{c}{\textbf{COSMU}}     \\ \hline
\multicolumn{1}{c|}{\textbf{CD}}     & 1.346              & 1.352               & 1.326                & \textbf{1.304}      \\ 
\multicolumn{1}{c|}{\textbf{Normal}} & .1523              & .1529               & .1503                & \textbf{.1475}      \\ 
\multicolumn{1}{c|}{\textbf{P2S}}    & 1.332              & 1.279               & 1.308                & \textbf{1.279}     \\


\end{tabular}           


==> tables/comparisons.tex <==
\begin{tabular}{c|cccc}

                                       &    \multicolumn{1}{c|}{\textbf{Methods}}        & \multicolumn{1}{c|}{\textbf{CD}}    & \multicolumn{1}{c|}{\textbf{Normal}} & \multicolumn{1}{c}{\textbf{P2S}}   \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{\textit{1 view}}}}} & \multicolumn{1}{c|}{PiFU~\cite{saito2019pifu}  }      & 1.698          & .1785           & 1.659          \\  
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{SuRS~\cite{SuRSECCV2022}    }    & 1.573          & .1693           & 1.554          \\ 
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{Baseline}    & 1.566          & .1732           & 1.570          \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{\textit{2 views}}}}} & \multicolumn{1}{c|}{PiFu-HD~\cite{saito2020pifuhd}  }   & 1.501          & .1663           & 1.512          \\ 
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{ICON~\cite{ICONCVPR2022}}        & 1.474          & .1695           & 1.463          \\ 
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{ECON~\cite{xiu2023econ}  }      & 1.368          & .1632           & \color[HTML]{3531FF}{1.365}          \\ 
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{COSMU-2 }    & \color[HTML]{3531FF}{1.355}          & \color[HTML]{3531FF}{.1593}           & 1.373          \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{\textit{4 views}}}}} & \multicolumn{1}{c|}{Multi-PaMIR~\cite{zheng2021pamir}} & 1.401          & .1650           & 1.385          \\ 
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{MVP~\cite{zhu2022mvp}}         & 1.348          & .1558           & 1.365          \\ 
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{COSMU}      & \color[HTML]{FF0000}{\textbf{1.304}} & \color[HTML]{FF0000}{\textbf{.1475}}  & \color[HTML]{FF0000}{\textbf{1.279}}

\end{tabular}
